VADIS: A Visual Analytics Pipeline for Dynamic Document Representation and Information-Seeking

In the biomedical domain, visualizing the document embeddings of an extensive corpus has been widely used in information-seeking tasks. However, three key challenges with existing visualizations make it difficult for clinicians to find information efficiently. First, the document embeddings used in these visualizations are generated statically by pretrained language models, which cannot adapt to the user's evolving interest. Second, existing document visualization techniques cannot effectively display how the documents are relevant to users' interest, making it difficult for users to identify the most pertinent information. Third, existing embedding generation and visualization processes suffer from a lack of interpretability, making it difficult to understand, trust and use the result for decision-making. In this paper, we present a novel visual analytics pipeline for user driven document representation and iterative information seeking (VADIS). VADIS introduces a prompt-based attention model (PAM) that generates dynamic document embedding and document relevance adjusted to the user's query. To effectively visualize these two pieces of information, we design a new document map that leverages a circular grid layout to display documents based on both their relevance to the query and the semantic similarity. Additionally, to improve the interpretability, we introduce a corpus-level attention visualization method to improve the user's understanding of the model focus and to enable the users to identify potential oversight. This visualization, in turn, empowers users to refine, update and introduce new queries, thereby facilitating a dynamic and iterative information-seeking experience. We evaluated VADIS quantitatively and qualitatively on a real-world dataset of biomedical research papers to demonstrate its effectiveness.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> tex/5System.tex <==
\vspace{-1mm}
\section{Visual Analytics System: \sysname{}}
Building on the capabilities of \modelshort{} to generate document embedding based on customized perspectives, \sysname{} is designed as a visual analytics system that facilitates flexible exploration of documents from multi-perspectives and knowledge synthesis. In this section, we first introduce the design philosophy of notecards, then illustrate the details of the interface and interactions employed. 
% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{figures/PerspectoCards_datamodel.pdf}
%     % \includegraphics[width=\linewidth]{figures/datamodel_case.pdf}
%     \caption{Illustration of the data model of \sysname{}, $[a, b, c, d...]$ are documents loaded in from document loader, $[e^{p_i}_a, e^{p_i}_b, ...]$ are prompt-based embedding generated on eaech notecard.}
%     \label{fig:datamodel}
% \end{figure*}
\vspace{-2mm}
\subsection{Design Philosophy}
In \sysname{}, the adoption of notecards as the primary design element stems from the belief that a flexible and interconnected approach is crucial for effective information-seeking. 
% In this context, notecards are virtual cards designed to intuitively store, visualize, and connect pieces of information in a flexible manner.
In this context, notecards are virtual cards that hold PAM-generated visualizations and associated documents. Each notecard represents a group of documents and their perspective information generated by PAM, such as the embedding.
% Notecards, in our context, are virtual cards used to store, explore, and synthesize insights from multiple perspectives. 
Inspired by the slip-box method, there are three key advantages of notecards that make them an ideal choice for our system design. We include the section number at the end of each philosophy to a detailed case study that demonstrates it in action.

\emph{DP1. Flexibility}: Notecards enable users to explore various perspectives and ideas without being constrained by a rigid workflow. Users can easily create new notecards to explore the corpus with emerging perspectives without disrupting existing notecards and their connections. (Section \ref{case-1}). 

% \emph{Scalability: } A notecard-based system allows for the seamless integration of new information as the research progresses. User can easily create new notecards to accommodate emerging insights and perspectives without disrupting existing notecards and their connections. 

\emph{DP2. Connection and synthesis}: Notecards facilitate the identification of connections and relationships between perspectives. This feature enables users to synthesize information from multiple notecards, each representing a different perspective, and uncover the interplay between these perspectives. Furthermore, users can also analyze the relationships between documents from different notecards under a new perspective, which can lead to a deeper understanding of the content (Section \ref{case-2}, \ref{case-3}, \ref{case-4})

\emph{DP3. Ease of use, organize, and showcase}: The concept of notecards is familiar and easy to understand, making the system accessible to users with varying levels of expertise. Naturally, notecards have two sides, which our dual-sided design takes advantage of, allowing users to view and interact with different types of information on each side. Furthermore, notecards can be collected and displayed on a virtual bulletin board, enabling users to organize and showcase their findings in a coherent and visually appealing manner. This simplicity and versatile features reduce the learning curve and allow users to quickly grasp the system's core functionality and focus on their research (Section \ref{case-4}).

In contrast to this philosophy, existing systems often fall short of embracing the flexibility and adaptability of a notecard-based approach. Constrained by static interfaces or predefined structures, they fail to support the dynamic, interconnected nature of information seeking. \sysname{} tackles the limitations of traditional systems by leveraging the unique advantages of notecards and \modelshort{}, providing a more comprehensive and intuitive solution for users.
% Flexibility: Notecards enable users to explore various perspectives and ideas without being constrained by a rigid structure. Users can create, arrange, and connect notecards as they see fit, allowing for a more organic and adaptable research process.

% Scalability: The notecard-based system allows for seamless integration of new information as the research progresses. Users can easily create new notecards to accommodate emerging insights and perspectives without disrupting their existing organizational structure.

% Connection and synthesis: Notecards facilitate the identification of connections and relationships between seemingly disparate ideas, enabling users to synthesize information and derive new insights from their research. This interconnected web of notecards encourages the discovery of patterns and trends that might have otherwise been overlooked.

% Ease of use: The concept of notecards is familiar and easy to understand, making the system accessible to users with varying levels of expertise. This simplicity reduces the learning curve, allowing users to quickly grasp the system's core functionality and focus on their


% Based on the two requirements (\textbf{R2, R3}) identified through the requirement analysis, we propose the following design tasks to address the challenges in information seeking:

% \emph{DP1. Develop an intuitive interface for customizing information-seeking pipelines} (\textbf{R2}). \sysname{} should involve an interface that allows for intuitive customization of the information-seeking pipeline. The interface should enable users to easily create and modify their pipeline and explore different perspectives as their understanding evolves. 
% Considering that researchers often need to view the distribution of multiple perspectives simultaneously to gain a comprehensive understanding of the corpus. Therefore, the interface should enable users to easily create and arrange multiple visualizations, allowing them to explore and compare different perspectives concurrently. %(create and arrange can lead to highlight sync functions)

% % Therefore the interface should include a dedicated ``insights board" feature, which allows users to select and organize key notecards in a unified space, similar to a physical bulletin board where researchers pin crucial information. This design encourages better information management, promotes the synthesis of findings across various perspectives, and enables more efficient comparisons.
% % To cater to the evolving needs of clinicians during the systematic review process, our first design task involves creating an interface that allows for intuitive customization of the information-seeking pipeline. The interface should enable users to easily modify their pipeline and explore different perspectives as their understanding evolves. It is important to consider that researchers often need to view the distribution of multiple perspectives simultaneously to gain a comprehensive understanding of the subject. Therefore, the interface should enable users to easily create and arrange multiple visualizations, allowing them to explore and compare different perspectives concurrently.

% \emph{DP2. Design an intuitive and versatile component for the major interface} (\textbf{R2}). \sysname{} should create a user-friendly component as the main component that supports visualizations, user interactions, and the annotations of findings and ideas. The component should allow users to access and manage the underlying data, as well as export data as needed. Additionally, the interface should incorporate logical operations that enable users to summarize or compare information across different notecards, facilitating a more comprehensive understanding of the research landscape. 
% % By focusing on these design aspects, we aim to create a versatile and adaptable component that effectively supports users throughout their information-seeking journey in the biomedical domain.
% % The goal is to develop a back side that facilitates data management, analysis, and prompt-based operations, providing users with direct access to underlying data and tools to enhance the efficiency and flexibility of their information-seeking process.

% \emph{DP3. Support efficient management and retrieval of insights} (\textbf{R3}). \sysname{} should provide users an effective way to manage and retrieve key insights generated throughout the information-seeking process. As the process evolves with many cards created, the system should allow users to collect cards for organization, search cards to retrieve the existing findings, and display them in a clean and organized manner for better synthesis and visual comparison. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/dual-sided-notecard.pdf}
    \caption{Dual-sided notecard with interactive frontside and action-oriented backside. }
    \vspace{-3mm}
    \label{fig:dual-sided-notecard}
\end{figure}
\vspace{-1mm}
\subsection{Design of Dual-sided Notecard}
% To create a more effective and user-friendly interface (\emph{DP2}), 
We design a dual-sided \emph{notecard} (Figure \ref{fig:dual-sided-notecard}) as the primary interface that supports visual exploration, user annotations, and management of the underlying data. Specifically, each notecard involves:

\textbf{Action-oriented back side}. The back side of the notecard serves as a hub for document management. Users can access data sources, export data, trigger prompt-based encoding, display the documents' relevance score, and filter documents based on the score.(Figure \ref{fig:dual-sided-notecard}-d). The motivation behind including documents within notecards lies in the fact that every finding originates from documents. Even though users might derive insights from visualizations, having the original data in each notecard enables users to easily trace the source of information and maintain context. This design grants users direct access to underlying data, enhancing the flexibility of their information-seeking process.

\textbf{Interactive front side}. The front side of the notecard is designed to facilitate the interactive exploration of documents from various perspectives. Users can incorporate three visualizations generated with \modelshort{} to delve into different levels of detail (Figure \ref{fig:dual-sided-notecard}-b), such as examining document distributions based on specific perspectives (document map), identifying the tokens of each document that receive the most attention under a particular prompt (context heat-map), and comparing documents from diverse sources (multi-category view). Specifically: 
% To facilitate the active engagement of users with their research findings, the front side of the notecard reserves a space for annotations and insights (Figure \ref{fig:dual-sided-notecard}-c), where users can record their thoughts, observations, and evolving understanding of the topic.
% Overall, the front side interactivity space allows users to explore document distributions, take notes and gain insights into the research landscape from various perspectives. 
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/cardtypes.pdf}
    \vspace{-7mm}
    \caption{Various type of card and functions notecard can perform}
    \vspace{-5mm}
    \label{fig:cardtypes}
\end{figure}

% \textbf{Visualizations generated with PAM} Front side of notecards incorporates three different visualizations generated with PAM's output, designed to facilitate users' understanding of documents from various perspectives and levels of detail. 
 
\emph{Document map} is a scatter plot that displays the distribution of documents based on a specific perspective (Figure \ref{fig:teaser}-$n_1$). Each dot represents a document embedding generated with \modelshort{}. We apply t-SNE to project the document embeddings from 768D into a 2D space. To make it more straightforward to clinicians, we apply k-means to cluster the embedding where the number of k is a user-defined parameter. We use the Elbow method \cite{elbow} to figure out the best k-value as default but allow users to modify or simply lasso groups of documents as their desired cluster. When displaying categorization results, each document category is assigned a distinct color. Additionally, by leveraging the document map and PAM, users can compare different groups of documents from various sources under specific perspectives. For example, one could compare two groups of studies to determine whether they examine the same population or treatment. The document map then highlights each data source with a unique color, enabling users to easily identify and differentiate between the groups. Users can also employ lasso selection directly on the document map to choose a group of documents for further analysis, providing a flexible approach for exploration and comparison of information from multiple perspectives.

\emph{Context Heat-map}
is designed to visualize the attention score that each token receives during the prompt-based embedding generation process (Figure \ref{fig:teaser}-$c_2$).
The context heat map utilizes the attention score of each token within a document and visualizes the distribution of attention scores following the principles of a heat map, enabling users to observe the attention distribution within a specific document. 
This visualization can help user understand what the model is focusing on and gain more confidence in the results.

\emph{Multi-Category View} 
present the distribution of documents across different perspectives by leveraging the concept of parallel coordinates. Each column represents a specific prompt, displaying categorization groups, with the column's height corresponding to the category's size. Documents are represented by lines that flow through multiple dimensions, illustrating their position in different categories. The size of the ribbons connecting the columns reveals the relationships between categories, offering insights into how documents are related or distinct across various perspectives. This comprehensive representation facilitates the exploration and comparison of documents from multiple angles, allowing users to gain an in-depth understanding of the corpus.

To facilitate the active engagement of users with their findings, the front side of the notecard reserves a space for annotations and insights (Figure \ref{fig:dual-sided-notecard}-c), where users can record their thoughts, observations, and evolving understanding of the topic.
Overall, the front side interactivity space allows users to explore document distributions, take notes and gain insights into the research landscape from various perspectives. 
% \emph{Document Map} 
% is a scatter plot that displays the distribution of documents based on a specific perspective (Figure \ref{fig:cardtypes}-a). Each dot represents a document embedding generated with \modelshort{}. We apply t-SNE to project the document embeddings from 769D into a 2D space. When displaying categorization results, each document category is assigned a distinct color. Additionally, when comparing different groups of documents from various sources, the document map highlights each data source with a unique color. Users can also employ lasso selection directly on the document map to choose a group of documents for further analysis.

% \emph{Context Heat-map}
% is designed to visualize token-level information, specifically highlighting which tokens or token spans receive the most attention during the prompt-based embedding generation process.
% The context heat map utilizes the attention score of each token within a document and visualizes the distribution of attention scores following the principles of a heat map, enabling users to observe the attention distribution within a specific document. 
% This visualization can help domain experts understand what the model is focusing on and gain more confidence in the results.
% % Simultaneously, to alleviate the burden of understanding the focus of each group of articles under a given perspective, the token map extracts the most attentive tokens from each document and aligns them in a grid layout. To achieve this, we employed an algorithm called RC-SOM\cite{tu2022phrasemap}, which maps each article's most attentive tokens to a position on a grid in a manner that maximizes the preservation of their similarities in the original document map.

% \emph{Multi-Category View}
%  leverages the concept of parallel coordinates to represent the distribution of documents across different perspectives. Each column represents a specific prompt, displaying categorization groups, with the column's height corresponding to the category's size. Documents are represented by lines that flow through multiple dimensions, illustrating their position in different categories. The size of the ribbons connecting the columns reveals the relationships between categories, offering insights into how documents are related or distinct across various perspectives. This comprehensive representation facilitates the exploration and comparison of documents from multiple angles, allowing users to gain an in-depth understanding of the corpus.


\textbf{Indexed and searchable content: }inside an information-seeking process, users may create numerous cards to delve into diverse aspects of the corpus. To ensure that these cards remain accessible and relevant throughout the information-seeking process (\emph{R3}), \sysname{} involves a search feature that indexes the content of each notecard, including the user's prompts, notes, and the most attentive tokens extracted based on the prompt. 
\vspace{-1mm}
\subsection{Connections Between Notecards}
% As researchers engage with notecards during their exploration, the connections between these notecards become crucial for facilitating insights generation, allowing them to dive deeper into specific subsets of information and synthesize findings from multiple perspectives. 
Inspired by traditional notetaking, researchers create connections between notecards by referencing or annotating to reflect their relationships. \sysname{} leverages the advantages of virtual notecards and supports three primary types of connections that cater to the diverse needs and goals of researchers:

\emph{Exploratory Connection}: Similar to how researchers might connect notecards together to indicate a relationship between the contents, our system enables users to create directed connections between virtual notecards for diving deeper into specific subsets of information. These virtual connections transfer a specific subset of data, such as user-selected groups, lassoed documents, or a particular category of articles after performing PAM encoding and categorization (Figure \ref{fig:cardtypes}-a).

\emph{Synthesis Connection}: As with physical notetaking, where researchers may combine notecards to synthesize insights from different perspectives, \sysname{} promotes the integration of findings from multiple research angles. The connections between notecards, in this case, enable data tracking as data sources are merged along with their respective perspectives. This functionality allows researchers to compare data from multiple groups within a new perspective (Figure \ref{fig:cardtypes}-b) or to examine the distribution of merged data across various perspectives (Figure \ref{fig:cardtypes}-c). Ultimately, this leads to the discovery of new insights and fosters a more comprehensive understanding of the research landscape.

\emph{Reference Connection}: Inspired by the practice of marking or bookmarking physical notes for later reference, \sysname{} support reference connection serves as a way to create reminders or flag notecards for future review. Unlike the other connection types, Reference Connections do not involve data flow between the linked cards. Instead, they simply provide an easy way for researchers to keep track of relevant notecards and ensure that they can quickly locate and revisit important information at a later time.
% \textbf{Data operations in connections:} 
% when a notecard is created and connected to a prior element, the data or selected portion of data from the element is transmitted to the notecard (Figure \ref{fig:datamodel}-a,b), the data includes information of each document, as well as the embeddings generated in each notecard for different prompts. Users can view document metadata on the back side with a data table view (Figure \ref{fig:teaser}-e). Initiating the prompt-based retrieval and encoding process involves editing the notecard's title (Figure \ref{fig:teaser}-e) with a natural language query ending in a question mark "?". \red{why these operations are not included in the back side?} Users can then flip the notecard to view the document map on the front side, add visualizations for different detail levels, and export selected documents for further analysis.
% When a notecard receives data from multiple sources, users can either \emph{merge} the data to examine document distributions from multiple perspectives, leveraging the proposed multi-category view, or compare the differences by assigning distinct visual parameters to highlight various sources. This facilitates efficient comparison of document groups based on a specific perspective during the information-seeking process.

\vspace{-1mm}
\subsection{Information-Seeking with Notecards}
With the design of a dual-sided notecard, the information-seeking pipeline in \sysname{} is conceptualized as a data flow diagram, with a document loader serving as the foundation for loading corpus data. Each node in this pipeline represents a notecard that can perform various tasks, such as PAM-based exploration, comparison, basic data storage, or even serving as a dedicated space for note-taking without any associated data. To facilitate seamless data flow, every notecard is equipped with two ports dedicated to data inflow and outflow, along with an additional two ports for reference connections that do not involve data transfer. This flexible and versatile design ensures that users can easily utilize any temporary notecard as a starting point for initiating a new information-seeking process, enabling a dynamic and efficient research experience tailored to the user's specific interests.

\vspace{-1mm}
\subsection{Canvas Mode and Insight Board Mode}
\sysname{} supports two distinct modes to cater to the diverse needs of users during their research process: \emph{Canvas Mode} serves as the primary mode, enabling users to create notecards for exploration, comparison, and synthesis of findings. This mode provides a flexible and adaptable space where researchers can freely interact with the notecards and their connections, facilitating a dynamic information-seeking process. \emph{Insight Board Mode} takes inspiration from the traditional bulletin board, providing a clean and focused dashboard for presenting the user's findings. All links and ports are hidden in this mode, allowing users to concentrate solely on the pinned notecards. The Insight Board Mode encourages better information management, promotes the synthesis of findings across various perspectives, and enables more efficient comparisons between insights. 
% By switching between these two modes, users can seamlessly transition from an exploratory process to a more organized and structured presentation of their findings.
\vspace{-1mm}
\subsection{Interactions Employed}
\sysname{} is equipped with intuitive interactions to support users to flexibly construct and keep track of their information-seeking pipeline. As illustrated in Figure \ref{fig:teaser}. Users can create an information-seeking process on the Canvas mode as follows: (1) create notecards, resize, and reposition notes in an intuitive drag-and-drop manner. (2) Hold and drag data ports of different notecards to create a link for transmitting a document set. (3) Stack up each notecard to card collections to organize and categorize insights. (4) retrieve the previous findings and insights by leveraging the notecards' content indexing and search functions. Through case studies and domain experts' feedback, we demonstrate the effectiveness and usability of these interactions in facilitating an effective and intuitive information-seeking process.

==> tex/8_supplymental.tex <==
\section*{Supplemental Materials}
\label{sec:supplemental_materials}

\subsection*{Efficiency Analysis of PAM}

Our model is being trained and tested on Nvidia Tesla V100 GPU for prompt-based document encoding tasks. We report the time cost of the preprocessing stage in Table \ref{tab:time}. The offline represents the preprocessing stage where each document goes through the document encoder and generates token embeddings with $E_D(\cdot)$; the online stage refers to the generation of prompt embedding, prompt-based attention, and the prompt-based embedding, based on the fact that the preprocessing has already finished and the token embedding of each document has been saved. In order to test the efficiency of PAM, we construct two test datasets from four question-answering datasets with 1K and 5K samples. The results demonstrate that PAM can handle a large number of documents at a near real-time speed, demonstrating the efficiency and scalability of PAM. 

\begin{table}[hbt!]
\caption{Time cost of encoding documents in the test dataset. Average length of document is 153 tokens}
  \vspace{2mm}
  
	\centering%
  \begin{tabu}{%
	l|
	c|
	c
	}
 \hline
  \toprule
  {Operation} & {Offline} & {Online}\\
 \hline
  \midrule
  Per Document Encoding $E_D(\cdot)$ & 1.6ms & - \\
  Per Prompt Encoding $E_P(\cdot)$  & - & 0.5ms \\ 
  Prompt-based Encoding(1,000) & - & 830ms \\
  Prompt-based Encoding(5,000) & - & 4,970ms\\ 
%   Retrieval 
  \bottomrule
    \hline
  \end{tabu}%
   
   \label{tab:time}
\end{table}

\subsection*{Ablation Study}
While our primary focus is on the biomedical domain, and emrQA is most relevant, incorporating general datasets such as SQuAD, TriviaQA, and Natural Questions is still beneficial since many clinical queries are expressed in general question formats, like ``what's the population being studied," which can be learned from general QA datasets. This approach enables the model to better locate relevant information across various contexts. We provide a detailed performance analysis with the involvement of different training datasets in the supplemental material.
We conducted an ablation study to analyze the necessity of training on both the biomedical domain question-answering dataset and the general QA datasets. The results are shown in Table \ref{tab:emrqa}. We report the accuracy of retrieval on the emrQA dataset as biomedical is our central domain. The result indicates that training on general datasets can also increase the accuracy of PAM with domain-specific questions.

\begin{table}[h] \small
	\centering%
  \caption{Performance of PAM in doing document retrieval with relevance score }
  \begin{tabu}{%
	l|
	c|
	c
	}
    \hline
  \toprule
  {Training/setting} & {emrQA@Top10} & {emrQA@Top20}\\
 \hline
  \midrule
  emrQA & 63.1 & 69.2\\
  emrQA+TriviaQA & 66.1 & 77.7 \\
  emrQA+TriviaQA+SQuAD & 68.9 & 73.2\\ 
  emrQA+All* & \textbf{70.1} & \textbf{79.6} \\
%   Retrieval 
\hline
  \bottomrule
 
  \end{tabu}%
   \vspace{2mm}
  
%   \vspace{-6mm}
\label{tab:emrqa}
\end{table}

